Data Quality Antipatterns for Software Analytics

Background: Data quality is vital in software analytics, particularly for machine learning (ML) applications like software defect prediction (SDP). Despite the widespread use of ML in software engineering, the effect of data quality antipatterns on these models remains underexplored. Objective: This study develops a taxonomy of ML-specific data quality antipatterns and assesses their impact on software analytics models' performance and interpretation. Methods: We identified eight types and 14 sub-types of ML-specific data quality antipatterns through a literature review. We conducted experiments to determine the prevalence of these antipatterns in SDP data (RQ1), assess how cleaning order affects model performance (RQ2), evaluate the impact of antipattern removal on performance (RQ3), and examine the consistency of interpretation from models built with different antipatterns (RQ4). Results: In our SDP case study, we identified nine antipatterns. Over 90% of these overlapped at both row and column levels, complicating cleaning prioritization and risking excessive data removal. The order of cleaning significantly impacts ML model performance, with neural networks being more resilient to cleaning order changes than simpler models like logistic regression. Antipatterns such as Tailed Distributions and Class Overlap show a statistically significant correlation with performance metrics when other antipatterns are cleaned. Models built with different antipatterns showed moderate consistency in interpretation results. Conclusion: The cleaning order of different antipatterns impacts ML model performance. Five antipatterns have a statistically significant correlation with model performance when others are cleaned. Additionally, model interpretation is moderately affected by different data quality antipatterns.

==> Introduction.tex <==
\section{Introduction}\label{sec:intro}

Machine Learning (ML) has been widely adopted in various domains of software analytics, including software defect prediction, technical debt identification, and effort estimation~\cite{menzies2010defect,tsoukalas2021machine,zimmermann2009cross,kamei2012large,ghotra2015revisiting}. These applications leverage ML to make key decisions, such as predicting future bugs, identifying problematic code, or estimating the required effort for software projects. In the domain of software analytics, data for models typically originates from software project repositories, issue tracking systems, and code commit histories, providing real-time and historical insights into software development practices. The users of these ML models expect not only high precision (for identification of specific issues) and recall (for ensuring no potential problems are overlooked), but also rely on these models for critical decision-making in software development and maintenance~\cite{tantithamthavorn2018experience,lyu2021empirical}. 

Apart from the choice of learning algorithm, hyperparameter tuning or embedding, the reliability of these decisions heavily depends on the quality of the data used to train the ML models~\cite{domingos2012few,tantithamthavorn2015impact,shepperd2013data}. Indeed, even if the code building the ML model is of high quality and is highly optimized, if the underlying data is flawed, the resulting model will be ineffective and potentially misleading. Unlike traditional software, where requirements are embedded as business logic encapsulated in software code, the requirements of ML models are embedded within the data itself. For example, to train a classifier distinguishing between cats and dogs, the training data must consist of accurate images of cats and dogs. If the dataset includes mislabeled images (e.g., an image of a rabbit labeled as a dog), the trained model will be compromised. Thus, the requirements of ML models are inherently tied to the quality and correctness of the data, making data an essential asset that determines the quality of the trained ML model~\cite{budach2022effects}.

Data being an important ML asset comes with its own suite of issues. While data quality issues are a recognized problem that compromises the quality of model training data, ``data quality antipatterns" are an important subset of such issues that could become problematic under certain circumstances. Similar to code antipatterns, their presence is not a direct indication of bugs or incorrect behavior, yet they can potentially compromise other qualities of ML models such as model performance and model interpretation. 
For example, class overlap occurs when samples with different classes have highly overlapping feature space, which may complicate their classification~\cite{kocaguneli2011exploiting}. Removing these points may help clarify class boundaries but could perhaps lose valuable information determining class boundaries thereby compromising the model learning. Similarly, on one hand, removing correlated \& redundant features reduces data (data loss can degrade performance~\cite{halevy2009unreasonable}), but on the other hand render interpretation results inaccurate~\cite{}. Another example is the presence of outliers, extreme values deviating from other observations, can skew model training and generalization but might not impact resilient learners. Literature~\cite{shepperd2013data,sharma2022performance,breck2019data,vzliobaite2016overview,chen2018tackling,denil2010overlap,vuttipittayamongkol2021class,gong2019empirical,johnson2019survey,yang2020rethinking,ali2019imbalance,daoud2017multicollinearity} has identified that such antipatterns can significantly affect the performance of software analytics ML models. For instance, while checking the impact of different bug labeling techniques on the performance of defect prediction models, Yatish et al.~\cite{yatish2019mining} obtained a 3\% to 5\% boost in AUC by correcting labels for defect classification models. Similarly, Gong et al.~\cite{gong2019empirical} observed a slight boost in AUC by removing data points having overlapping classes.

% para
% While prior studies have examined these antipatterns, they did so in isolation, which may not provide a comprehensive understanding of their overall impact~\cite{chen2018tackling,mcintosh2016empirical,shepperd2013data}. For instance, in the above example of defect classification by Yatish et al.~\cite{yatish2019mining}, the authors did not consider the impact of class overlap or class imbalance. 

Similarly, research~\cite{shepperd2013data,sharma2022performance,breck2019data,vzliobaite2016overview,chen2018tackling,denil2010overlap,vuttipittayamongkol2021class,gong2019empirical,ali2019imbalance,daoud2017multicollinearity} cleans data using ``generic'' cleaning techniques like removal of null values, a comprehensive suite of cleaning techniques is not applied. Perhaps an obvious reason for this is the lack of a well-defined taxonomy of data quality antipatterns. Although some antipatterns like tailed distributions~\cite{hynes2017data}, distribution shift~\cite{hynes2017data}, or feature-row imbalance~\cite{Debie} exist in general research, they have not been studied in the context of software analytics, despite the widespread use of ML in this field. Perhaps software analytics research missed such antipatterns assuming them to be harmless, without having an empirical understanding of their real impact. 

Moreover, prior research has typically 1) studied these antipatterns in isolation, neglecting the possibility that multiple antipatterns can coexist and interact (e.g., in the above example of defect classification by Yatish et al.~\cite{yatish2019mining}, the authors did not consider the impact of class overlap or class imbalance); and 2) not address potential reasons for retaining antipatterns as not all antipatterns can be significantly harmful, but their removal will incur substantial costs, i.e., valueable data might be removed or imputed during the data cleaning processes. Given that some data is better than less data, especially in scenarios with limited data availability, the performance degradation costs can be non-trivial. 

Data pipelines are complex and can spread across multiple servers, machines, or IoT devices across various geolocations. For instance, if a machine reading sensor data already cleans the data before transmitting it to the central server for ML model development, the data might need selective cleaning, at the server level. However, the understanding of the systematic addressing of antipatterns or order of their removal missing.

This lack of understanding makes data scientists experiment with multiple data configurations, causing overhead in the process of ML pipeline development. The crippling effects of a lack of structured understanding of addressing data quality antipatterns not only manifest in data-related issues, but also extend to software maintenance related-issues, leading to experimentation pipeline jungles and dead code paths, unclean git branches, hampering code maintenance.

This scenario highlights the primary motivation for our work, which is to investigate the order and impact of addressing antipatterns given circumstances where keeping antipatterns might be justified due to the high cost of their removal, along  with explicitly evaluating the impact of one antipattern, where we aim to remove overlapping effects and assess an antipattern without it being influenced by others. This approach will help practitioners focus on prioritizing critical antipatterns, especially in scenarios where partial cleaning has been done, potentially reducing the overall effort required to enhance data quality in software analytics models and avoiding the performance degradation that comes with antipattern removal.

Hence, in this study, we address these challenges by developing a taxonomy based on general literature on data quality, and identifying eight ML-specific data quality antipatterns, i.e., \textit{Schema Violations, Data Miscoding, Inconsistent Representation, Data Distribution Antipatterns, Packaging Antipatterns, Row-Feature Imabalance, Label Antipatterns}, and \textit{Correlation \& Redundancy}, and 14 antipattern sub-types. This taxonomy provides a structured understanding of the potential issues that could affect data quality not only in software analytics, but other fields as well.

We then use Software Defect Prediction (SDP) as a case study to understand the impact of these antipatterns on the performance and interpretation of software analytics models. This allows us to investigate these antipatterns in a practical, real-world context, and have a focused understanding of their implications on software analytics using a dataset widely used in research~\cite{rajapaksha2021sqaplanner,jiarpakdee2021practitioners,tong2019kernel,gong2021revisiting,moussa2022use,jiarpakdee2020empirical,wattanakriengkrai2020predicting,fu2022linevul}. SDP is particularly significant due to its widespread use in research and the criticality of its role in maintaining software quality. SDP datasets used in these studies have been reused extensively in the software analytics research community~\cite{menzies2010defect,jiarpakdee2021practitioners}, along with for ML benchmarking~\cite{ghotra2015revisiting,aleem2015benchmarking}. Therefore, understanding the impact of data quality antipatterns in the context of SDP can provide valuable insights that can be generalized to other areas of software analytics. 

Hence, operationalizing SDP models, comes with several practical real-world decisions including but not limited to the quality of data used to train the models. First, we need to determine whether the order of cleaning antipatterns could potentially affect the performance of the models, and, if so, find the optimal sequence for a more efficient and effective cleaning process. Second, we must assess the impact of antipatterns on model performance in a setting where other antipatterns are cleaned out. Understanding whether antipatterns interact is crucial to assess the severity of each antipattern and prioritize our cleaning efforts accordingly. This understanding is needed to determine if it is worth sacrificing data for cleaning when available data is sparse and the impact of these issues is not significant. In some cases, retaining more data, even with some quality issues, might be more beneficial than losing data to rigorous cleaning.

Finally, the interpretation of ML models is a crucial aspect of software analytics, especially when it comes to making informed decisions based on a ML model's predictions. For instance, in software defect prediction, understanding which features contribute most to a prediction can help developers focus their debugging efforts more effectively. Similarly, in effort estimation, interpreting the model can reveal which aspects of a project are likely to require the most resources, enabling better project planning and resource allocation. Prior studies have explored the impact of various factors such as learner characteristics, project specifics, hyperparameter tuning, and sampling randomness on interpretation results~\cite{lyu2021towards}, while overlooking the noise introduced by ``data quality''on the interpretation results of ML models. This gap in the literature presents an opportunity for further exploration and understanding, which we address in this study.

Overall, after establishing a taxonomy of eight antipatterns (\textit{Schema Violations, Data Miscoding, Inconsistent Representation, Data Distribution Antipatterns, Packaging Antipatterns, Row-Feature Imabalance, Label Antipatterns}, and \textit{Correlation \& Redundancy}), along with 14 sub-types of antipatterns, we study the following research questions (RQs) in our case study:
\begin{itemize}
    \item \textbf{\rqone} \\ 
    \textit{Results:} SDP data contains \textit{schema violations, correlated \& redundant features, distribution antipatterns (tailed and not normal distributions), mislabeling,} and \textit{duplicated data} antipatterns. We found no instances of \textit{data miscoding, missing values} or the \textit{data drift} antipattern in the studied data. 
    Antipatters also overlap within projects and co-exist both on the row and column level in the tabular data. On the row level, 94\% of the rows with more than one antipattern include \textit{mislabels} and \textit{class overlap}. On the column-level, 90\% of the columns having two antipatterns include correlated \& redundant features and tailed features.
    
    \item \textbf{\rqtwoone} \\ 
    \textit{Results:} The order of cleaning impacts model performance, with certain orders having more pronounced effects than others. Removing class overlaps before  transformation consistently boosts the performance across all learners, emphasizing the importance of performing transformation at the end. In contrast, sequences like filtering before transformation and mislabel correction before overlap removal show varied impacts depending on the learner; simplistic classifiers like  Logistic Regression significantly benefit from mislabel correction before class overlap correction, while DNN shows robustness in its capacity to be resilient to different orders of cleaning antipatterns.

    
    \item \textbf{\rqtwotwo} \\
    \textit{Results:} 
    Although introduction of five antipatterns (\textit{Tailed, Mislabel, Class Overlap, Class Imbalance, Correlation \& Redundancy}) has a statistically significant impact on the performance metrics, most antipatterns only introduce a negligible to small effect on model performance. Among the antipatterns having an impact, only the \textit{Tailed} and \textit{Class Overlap} antipatterns result in a medium or large effect on some of the performance metrics. Overall there is heavy variability in the impact of different antipatterns across different learners.
    
    \item \textbf{\rqthree} \\ 
    Models constructed from data with different antipatterns exhibit moderate consistency in interpretation. This enhances the body of research on model interpretation which previously identified factors that impact the interpretation results, such as learner characteristics, hyperparameter tuning, and sampling randomness.
    
\end{itemize}



Our study offers empirical guidance for software analytics practitioners, enabling them to make well-informed data cleaning decisions in a real world setting. Our results not only aid in prioritizing data cleaning activities but also urge practitioners to consider data quality\bram{people already know about this before?}\aadi{No: this is our novel insight.} as a factor while trusting the reliability of model interpretation results within the realm of SDP. Furthermore, data scientists, irrespective of their domain, can leverage our taxonomy to better understand and anticipate the real-world impacts of addressing antipatterns on the performance and interpretation of their machine learning models.

The remainder of the paper is organized as follows. Section~\ref{sec.lit} presents the relevant literature on data quality. Section~\ref{sec.back} explains the prestudy that summarizes the related work into a taxonomy of data quality antipatterns. Section~\ref{sec.casestudy} provides an overview of the case study setup along with a description of the case study parameters and various statistical tests used in this study. Section~\ref{sec.results} discusses the motivation, approach, and results for each of our research questions. Section~\ref{sec.threats} discusses threats to the validity of our study, while Section~\ref{sec.discussion} provides a discussion on our results. Section~\ref{sec.implications} provides the implications of our findings for researchers and practitioners, and finally, Section~\ref{sec.conclusion} concludes the paper.

==> Supplementary_Material/proxy_setup.tex <==
# Developer laptop setup <!-- omit in toc -->

This setup should be done in Huawei premises, since working from home requires [additional configuration](#working-from-home) and makes problem debugging harder.

After you laptop is properly setup, you should have:
- WSL 2 installed
- Proxy configured
- SSL certificates installed
- Docker installed
- Huawei mirrors being used whenever possible
- VSCode installed

**Disclaimer**: The instructions shown in this README are provided without any warranty and do not represent or replace Huawei's official instructions. Always double-check things with your supervisor and make sure that you adhere to the company's policies, rules, and guidelines. Happy coding!

# Table of contents <!-- omit in toc -->

- [Install WSL2](#install-wsl2)
- [Setup Ubuntu mirror](#setup-ubuntu-mirror)
- [Setup proxy](#setup-proxy)
- [Install SSL Certificates](#install-ssl-certificates)
  - [Producing the certificates](#producing-the-certificates)
  - [Installing the certificates](#installing-the-certificates)
  - [Making certificates available to other programs (special cases)](#making-certificates-available-to-other-programs-special-cases)
- [Install w3m to test connectivity and SSL](#install-w3m-to-test-connectivity-and-ssl)
- [Install Container Management Technology](#install-container-management-technology)
  - [Option1: Docker](#option1-docker)
  - [Option2: Podman and Podman Compose](#option2-podman-and-podman-compose)
- [Install VSCode](#install-vscode)
- [Install poetry and configure it to create .venv in project](#install-poetry-and-configure-it-to-create-venv-in-project)
- [Working from home](#working-from-home)


## Install WSL2

- Turn on WSL in the windows features:
$ Enable-WindowsOptionalFeature -Online -FeatureName Microsoft-Windows-Subsystem-Linux 

- Install WSL2 and a Ubuntu distribution with the following commands and restart your laptop. (https://learn.microsoft.com/en-us/windows/wsl/wsl-config)

```bash
# install wsl
wsl --install

# check the wsl version
wsl -v

# install lastest Ubuntu LTS as default disto
wsl --install -d ubuntu
```

[Optional] Install Windows Terminal and set it as the default terminal application. (https://learn.microsoft.com/en-us/windows/terminal/install)


**Note**: The instructions shown in this README.md apply for *developer laptop* only. If you are setting up WSL2 on a secure PC, then you likely formal permission from your supervisor. Check the following two URLs:
- http://3ms.huawei.com/hi/group/3764331/wiki_7183031.html
- https://spa.iright-t.huawei.com/#/wf/generalFilingApply?subCategoryCode=1316


## Setup Ubuntu mirror

Check instructions on `http://mirrors.tools.huawei.com`

Then:

```bash
sudo apt-get update
sudo apt-get upgrade
```

## Setup proxy

- A bash file with the following contents:

```bash
#!/bin/bash

# Reading values
PROXY_USER="g00639664"
read -s -p "Enter proxy password: " PROXY_PWD
echo

# Let's define our proxies
export http_proxy="http://$PROXY_USER:$PROXY_PWD@proxyca.huawei.com:8080"
export https_proxy="$http_proxy"
export ftp_proxy="$http_proxy"
export no_proxy=127.0.0.1,localhost,huawei.com,10.193.182.78

# For whatever reason, curl (and some other tools) search for uppercase  
# versions of these variables. So we'd better have them too:
export HTTP_PROXY="$http_proxy"
export HTTPS_PROXY="$https_proxy"
export FTP_PROXY="$ftp_proxy"
export NO_PROXY="$no_proxy"
```

The basic idea is: all traffic that is external to Huawei ("outside world") should go through the proxy. Analogously, internal Huawei websites and servers should be accessed directly (without the proxy).

**Note 1:** The IP `10.193.182.78` in `$no_proxy` is only relevant to the `Software 4.0` research project. That IP is the address of the Kingston1 server (a.k.a., testing server). If your research project accesses servers inside the Huawei network, make sure to add them to the `$no_proxy` variable.

**Note 2:** If you have special characters in your password, they need to escaped. Check [here](https://johndecember.com/html/spec/esccodes.html)

- Load this file using `source [the-script.sh]`. You may also add this line to your `.bashrc` file to ensure that these variables are always loaded in every bash session.

- Once proxy is setup, almost every Linux tool should work fine. Some specific tools however do require proper flags or configuration to work properly. For instance, if you are running `curl`, add the `-L` flag (to allow redirections).

## Install SSL Certificates

### Producing the certificates

Three certificates are needed in total: two for internal Huawei domains and one for external domains. To obtain these three certificates, do the following:
- Certificates for internal Huawei domain: From a Huawei Laptop/Desktop, visit a secure Huawei website (e.g., [CodeHub](https://codehub-g.huawei.com/workspace/projects)) using Chrome. Now, click on the `lock` icon right beside the url, then `Connection is secure`, then `Certificate is valid`. A new popup window will open. Click on the `Details` tab. Select `Huawei IT Root CA` and then click `Export`. Now just save the CRT file (no need to change any settings). Now select `HWIT Enterprise CA 1`, click `Export`, and save the CRT file.
- Certificate for external domains: The process is the same. However, now you need to visit an external website (e.g., [GitHub](https://github.com/openssl/openssl/actions)). The certificate that needs to be saved is called `Huawei Web Secure Internet Gateway CA`.

### Installing the certificates

Copy the three crt files to `/usr/local/share/ca-certificates` and run:

```bash
sudo update-ca-certificates
```

Make sure you see `3 added`. If you see that, it means that the SSL certificates have been successfully installed. Most unix applications will be able to automatically detect these certificates now and SSL problems should disappear (e.g., `self-signed certificate in chain` problems).

### Making certificates available to other programs (special cases)

Not every program running on Linux is able to automatically fetch/consume the certificates that we just installed. Two classic examples are JVM (Java virtual machine) and pip (python package installer).

**- Java**: The easiest way to make SSL certificates available to the JVM is to install the `ca-certificates-java` Ubuntu package:

```bash
sudo apt-get install ca-certificates-java
```

After this package is installed, running the `update-ca-certificates` command will also make all certificates available to the JVM (i.e., certs will be imported into the Java cert keystore).

**- Python's pip**: Python's pip: When running `pip` (or `pip3`), the certificates need to be provided via a `--cert` parameter (see [here](https://stackoverflow.com/a/26062583)). For instance, to install a package from an external domain (e.g., GitHub), the `Huawei Web Secure Internet Gateway CA` needs to be provided. On Ubuntu, all installed certificates can be found under `/etc/ssl/certs`. Example:

```bash
sudo pip3 --cert /etc/ssl/certs/huawei-web-secure-internet-gateway-ca.pem install https://github.com/containers/podman-compose/archive/devel.tar.gz
```

Certificates can also be made available to pip using environment variables. See [here](https://pip.pypa.io/en/stable/topics/https-certificates/#using-a-specific-certificate-store).


## Install w3m to test connectivity and SSL

To assist us in testing the proxy and SSL certificates, let's install `w3m` (a shell web browser):

```bash
sudo apt-get install w3m
```

To test whether Proxy and SSL certificates are working as desired, just try to visit the two following websites. You should be able to view the two websites without any error messages:

```bash
w3m https://codehub-g.huawei.com # internal website
w3m https://www.github.com # external website
```

## Install Container Management Technology

### Option1: Docker

- Follow online instructions here: https://docs.docker.com/engine/install/ubuntu/#install-using-the-repository

- Next, add the following contents to `C:\Windows\System32\drivers\etc\hosts` (open the file as Administrator):

```bash
# Added by Docker Desktop
10.213.123.121 host.docker.internal
10.213.123.121 gateway.docker.internal
# To allow the same kube context to work on the host and the container:
127.0.0.1 kubernetes.docker.internal
```

- Reboot the machine
- Open WSL2
- Do `cat /etc/hosts` and ensure that the changes we've just done to Windows's `host` file are reflected here

- Test docker with the following two commands: 

```bash
sudo docker pull httpd #To check if docker is able to download/pull images
sudo docker run hello-world #To test if docker can download/pull an image AND run a container
```

**Note:** If the test above fails, reach out to Gustavo (g00639664).

### Option2: Podman and Podman Compose

Podman is an alternative to docker. It's key feature is the ability to run 'rootless containers'. Podman offers the exact same commands as docker, since both implement the OCI (Open Container Initiative). It's popularity has increased substantially over the year. However, docker remains the de-facto choice for container management and has a much larger community around it.

- Podman is available from `Ubuntu 23.04` onwards. If you followed the WSL setup instructions, your Ubuntu version will be the latest LTS release. As of today (October 2023), the latest LTS release is `22.04`. Hence, the easieast way to install `podman` right now is to perform an in-place upgrade from `Ubuntu 22.04` to `23.04` (once `24.04 LTS` is out, this problem won't exist anymore). Instructions for in-place upgrade can be found [here](https://askubuntu.com/questions/1459438/how-to-upgrade-ubuntu-22-04-to-23-04).

- Once Ubuntu 23.04 or higher is installed, you can install podman directly from `apt` using `sudo apt-get install podman`.

- To allow podman to pull images without authentication, perform the following commands (more info [here](https://podman.io/docs/installation#add-configuration)):

```bash
sudo mkdir -p /etc/containers
sudo curl -L -o /etc/containers/registries.conf https://src.fedoraproject.org/rpms/containers-common/raw/main/f/registries.conf
sudo curl -L -o /etc/containers/policy.json https://src.fedoraproject.org/rpms/containers-common/raw/main/f/default-policy.json
```

- Test podman with the following two commands (if prompted to pick a registry, pick `docker.io`): 

```bash
podman pull httpd #To check if podman is able to download/pull images
podman run hello-world #To test if podman can download/pull an image AND run a container
```

- Install `podman-compose` by following the instructions from the [official repo](https://github.com/containers/podman-compose). `podman-compose` is 99% compatible with `docker-compose` (same API, same commands).

## Install VSCode

Follow instructions from the official website.

## Install poetry and configure it to create .venv in project

This ensures that VSCode can easily find your Python interpreter

- Install poetry using instructions from [official website](https://python-poetry.org/docs/#installation).
- Configure poetry to create .venv inside project (`virtualenvs.in-project`). See here `https://python-poetry.org/docs/configuration/`

## Working from home

Install wsl-vpnkit: `https://github.com/sakai135/wsl-vpnkit`


==> old/Introduction-OLD.tex <==




\section{Introduction}\label{sec:intro}



% General motivation
The widespread adoption of Machine Learning (ML) technology in software systems, calls for the need for quality assurance for ML software. At one end of the spectrum, ML software needs to adhere to all traditional software quality metrics, including functionality, readability, efficiency, security, and reliability. On the ``ML-specific`` side of the ML quality spectrum, an ML software needs to ahdere to the AI trust assessment metrics like Fairness, Trustworthiness, robustness~\cite{santhanam2020quality}. Finally, the predictions generated by an ML model are based on the data that is used to train the model, giving rise to the ``data quality'' aspect of the ML quality spectrum. The fit of an ML model is dependent on the quality of the data used to train it\cite{domingos2012few}. Since data is not a part of the software, but a mere ML artifact~\cite{idowu2022asset}, data quality calls for a separate level of scrutiny. This is also evidenced by the community of academics, industrial standardization bodies, and toolsmiths developers which heavily focus on data quality for ML. The International Standards Organization (ISO) has defined general data quality through standards such as ISO 8000-61: \textit{Data Quality management: Process reference model}. While SQuaRE metrics, defined under ISO/IEC 25024\footnote{\url{https://www.iso.org/standard/35749.html}} cover general aspects of data quality, such as accuracy, completeness, consistency, and credibility, however, fail to fully address the data quality needs for ML. On the tooling side, significant advancements have been made in data validation and cleaning. Caveness et al.'s TFDV tool~\cite{caveness2020tensorflow} offers a wide range of data validation capabilities, including the verification of data schema, the detection of data drift, and the visualization of features. Additionally, the DataPrep tool~\cite{dataprep} provides functionalities for visualizing data and removing inconsistently represented entities, such as country codes and phone numbers. Furthermore, the Holoclean tool~\cite{rekatsinas2017holoclean} is specifically designed to repair inconsistent datasets. These tools collectively contribute to improving the perceived quality of data used for various ML applications. While such tools are available for cleaning data, it is still not known whether a specific antipattern should be cleaned?\\
Along with such industrial tools, the data community around academic research have shown the impact of singular data quality antipatterns. For instance, antipatterns like overlapped classes~\cite{chen2018tackling,denil2010overlap,vuttipittayamongkol2021class,gong2019empirical}, correlated \& redundant variables~\cite{mcintosh2016empirical}, null and implausible values~\cite{shepperd2013data}, and labeling strategies~\cite{yatish2019mining}, have been extensively studied by the academic community. Although research has demonstrated the impact of individual data quality antipatterns, it is likely that multiple data quality antipatterns coexist in practice, due to which the prior research do not answer questions like: what is the impact of cleaning multiple antipatterns in different orders? what is the impact of an antipattern when the remaining ones have been cleaned out? \\
Additionally, model interpretation is crucial in ML for understanding complex models and their predictions, build trust in the model's decisions, detect biases, and identify errors. Yet, it remains unknown whether data quality antipatterns affect the interpretation of ML models, despite the widespread adoption of ML interpretation in the decision-making process~\cite{lyu2021towards,liu2022performance}. 
To answer such questions, we consider the case of software defect prediction (SDP). SDP is a technique used to estimate the likelihood of bugs in a specific file by analyzing both software and development process-based features. SDP is a well-established research area with a history of more than two decades due to which we leverate their dataset for our research.
In this paper, we first develop a taxonomy of seven ML-specific data quality antipatterns, i.e., \textit{Schema Violations, Data Miscoding, Inconsistent Representation, Data Distribution Antipatterns, Packaging Errors, Label Antipatterns}, and \textit{Correlation \& Redundancy}, that contain 12 antipatterns sub-types.
We then use software defect prediction (SDP) as a case study to understand the impact of data quality antipatterns on the performance and interpretation of ML models. In particular, we set out to answer the following research questions (RQs). \\
\begin{itemize}
    \item \textbf{\rqone} \\ 
    \textit{Results:} SDP data contains \textit{schema violations, correlated and redundant features, distribution antipatterns (tailed and not normal distributions), mislabeling,} and \textit{duplicated data} antipatterns. We found no instances of \textit{data miscoding, missing values} or the \textit{data drift} antipattern. On the row level, 94\% the rows which have more than one antipattern include \textit{mislabels} and \textit{class overlap}. On the column level, 90\% of the columns having two antipatterns include correlated \& redundant features and tailed features.
    
    \item \textbf{\rqtwoone} \\ 
    \textit{Results:} Order of cleaning antipatterns has no impact on the performance of the defect prediction models. An antipattern cleaning order pair (say Mislabel correction (\textit{Mi}) \rightarrow Class overlap correction (Ov)) would have better performance than its inverse order (Ov \rightarrow Mi) in only 50\% of the cases which is only random.
    
    \item \textbf{\rqtwotwo} \\
    \textit{Results:} Although five antipatterns (\textit{Tailed, Mislabel, Class Overlap, Class Imbalance, Correlation \& Redundancy}) have a statistically significant effect on performance metrics, most antipatterns only introduce a negligible to small effect on the model performance. Among the antipatterns, only the Tailed and Class Overlap result in a medium or large effect on some of the performance metrics.
    
    \item \textbf{\rqthree} \\ 
    Models built from data containing different antipatterns have a moderate interpretation consistency.
    
\end{itemize}


% \subsection{Paper Organization}
The remainder of the paper is organized as follows. Section~\ref{sec.back} explains the prestudy which summarizes the related work into a taxonomy of data quality antipatterns. Section~\ref{sec.casestudy} provides an overview of the case study setup along with a description of the case study parameters and various statistical tests used in this study. Section~\ref{sec.results} discusses the motivation, approach, and results for each of our research questions. \aadi{Gopi, is this order good?} Section~\ref{sec.lit} presents the relevant literature in data quality, while Section~\ref{sec.threats} discusses threats to the validity of our study. Section~\ref{sec.implications} provides the implications of our findings for researchers and practitioners, Section~\ref{sec.discussion} provides a discussion on our results, and finally, Section~\ref{sec.conclusion} concludes the paper.

==> old/main_TSE.tex <==
% \documentclass[conference]{IEEEtran}
% \IEEEoverridecommandlockouts

% for nemenyi
\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing}
% nemenyi end


% correcting citations
\usepackage[colorlinks,bookmarksopen,bookmarksnumbered,citecolor=red,urlcolor=red]{hyperref}
\usepackage{multirow} % added for merge cell in table
\usepackage{changepage}% to make table to left
\usepackage{hyperref} % for hyperlinks @ plotly and urls
\usepackage{soul} % strikeout
\usepackage[super]{nth}
\usepackage{adjustbox}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{url}
\usepackage[dvipsnames]{xcolor}

\usepackage{comment}
\newcommand\ytl[2]{
\parbox[b]{10em}{\hfill{\color{cyan}\bfseries\sffamily #1}~$\cdots\cdots$~}\makebox[0pt][c]{$\bullet$}\vrule\quad \parbox[c]{4.5cm}{\vspace{7pt}\color{red!40!black!80}\raggedright\sffamily #2.\\[7pt]}\\[-3pt]}

% summary box =================================================
\usepackage[most]{tcolorbox}
\definecolor{custom-gray}{cmyk}{0, 0, 0, 0.7, 1.00}
\newtcbtheorem[no counter]{Summary}{\hskip-0.97em}{enhanced,drop shadow={black!50!white},
 coltitle=white,
 top=0.15in,
 attach boxed title to top left=
 {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
 boxed title style={size=small,colback=custom-gray}
}{summary}


% for listing =================================================
\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{xcolor}
\usepackage[super]{nth}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle} 
%%%%%%% LISTING END



% RQs defined here =========
\newcommand\rqone[0]{RQ1: What is the prevalence of data quality antipatterns in software defect prediction data?}
    \newcommand\rqtwoone[0]{RQ2: How does the order of cleaning data quality antipatterns impact the model performance?}
\newcommand\rqtwotwo[0]{RQ3: How do data quality anti-patterns impact model performance?}
\newcommand{\rqthree}[0]{RQ4: How do data quality anti-patterns impact model interpretation?}

 
 % commenters defined here
\newcommand{\aadi}[1]{\textcolor{blue}{\textit{[Aadi says: #1]}}}
\newcommand{\dayi}[1]{\textcolor{green}{\textit{Dayi says: [#1]}}}
\newcommand{\gopi}[1]{\textcolor{green}{\textit{Gopi says: [#1]}}}
\newcommand{\ques}[1]{\textcolor{orange}{\textbf{\textit{Question for Dayi/Gopi: [#1]}}}}


\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{document}

\title{Data Quality Issues in Software Engineering: A Case Study of Software Defect Prediction}

\author{Aaditya~Bhatia \and Dayi~Lin \and Gopi~Krishan~Rajbahadur \and Zhen~Ming~(Jack)~Jiang

\IEEEcompsocitemizethanks{
    % \IEEEcompsocthanksitem Aaditya~Bhatia is with Software Analysis and Intelligence Lab (SAIL) School of Computing, Queen's University, Canada. E-mail: aaditya.bhatia@cs.queensu.ca\protect\\
    % \IEEEcompsocthanksitem Dayi~Lin and Gopi~Krishnan~Rajbahadur are  senior researchers at Huawei, Canada. E-mail: \{dayi.lin, Gopi.krishnan.rajbahadur1\}@huawei.com\protect\\
    %  \IEEEcompsocthanksitem Zhen Ming (Jack) Jiang 
    % is an Associate Professor and director of SCALE Lab, York University, Canada. E-mail: zmjiang@cse.yorku.ca\protect\\
    % \IEEEcompsocthanksitem Aaditya~Bhatia is the corresponding author
}
\maketitle


% \input{abstract}
\begin{IEEEkeywords}
Data~Quality, Machine~Learning  \end{IEEEkeywords}

\input{Introduction}
\input{Prestudy.tex}
\input{case_study}
\section{Research Questions}\label{sec.results}
    \input{rq1}\label{subsec.RQ1}
    \input{rq2_orders}\label{subsec.RQ2}
    \input{rq2_aps}\label{subsec.RQ3}
    \input{rq3}\label{subsec.RQ3}
\input{Threats}
\input{Conclusion}
\input{Discussion.tex}
\section{Data Availability}
All the scripts along with the mined data are provided in the replication package\footnote{Tentative g-drive (\url{}) will be replaced by a GitHub repository GitHub link replication package  will be provided after the publication.\aadi{do after getting 1st revision from GOPI/DAYI.}}


\bibliographystyle{IEEEtran}
\bibliography{references}
\include{Appendix}
\end{document}


==> old/old_RQ2_orders.tex <==
 Indeed, a data scientist/data engineer would face with these challenges, and they may come up with a ``locical'' explanation for cleaning multiple antipatterns. For instance, in the case of our dataset, we identified that ``Filtering''-based cleaning ought to be performed first. This is done so that the ``Transformation''-based cleaning has the correct dataset information. Next, we perform ``Mislabel'' correction so that ``Class-Overlap'' correction has the correct information of the response variable. Finally the ``Class Overlap'' correction is done at the end so that the distribution of the dataset which is to be used to train the model is the same distribution as that which is removed by class overlap. \\
 Nonetheless, our logic for cleaning does not apply for other dataset, neither do we have information of whether our identified ``logical'' order yields the best model metrics? Hence, through this research question, we wish to provide an empirical understanding to reserachers and practitioners for understanding of the impact of the order of cleaning antipatterns while building their ML models, by taking the case study of SDP dataset.



%  this was for before 2023

Amongst MO and OM, mislabel correction before overlap yields higher AUCs for all six classifiers. This is natural as the data size for MO is more. However this effect is more pronounced for classifiers having high degrees of freedom. In particular, NN, SVM and RF, have a higher impact of mislabel correction after class overlap which yeilded more data points. We suspect that this is due to classifiers having high DPF need more data points for training.


For the cases with class overlap not performed on mislabel correction, (i.e., all orders with \texttt{MO}) T\textbf{MO}F, TF\textbf{MO}, and FT\textbf{MO} have best performing AUCs for all six classifiers. While, F\textbf{MO}T has higher performing AUC ranks for 3/6 classifiers. We suspect this is the case because class overlap needs correct transformation as that used for the model building. The effect is pronounced in Dtree, NN, and LR. Naturally, \textbf{MO}FT and \textbf{MO}TF are will yeild similar AUCs. Both \textbf{MO}FT and \textbf{MO}TF have a lower AUC because class overlap did not have accurate data distribution as that of the model building process.\\

%==============================%===========
\begin{Summary}{Summary of RQ2}{}
While changing the cleaning order has an effect on the size of the training data. Class overlap needs accurate representation of data. This manifests in 1) lower training data size if class overlap has incorrect information of the response label; and 2) lower AUCs when class overlap has incorrect representation of the explanatory variables.
\end{Summary}
%==============================%===========


\subsubsection{Training Data Size}
\dayi{instead of size can have other metrics like similarity of dataset. some metrics that show difference between feautres. Drift? check for some other pkgs, that are less sensitive.}\aadi{to discuss/}

    \begin{figure}[!h]
          \centering
          \includegraphics[width=\columnwidth, keepaspectratio]{Images/Orders_trainSize.pdf}
          \caption{Size of the training data after cleaning via different cleaning orders. }
          \label{fig.orders.size}
    \end{figure}
    
\textbf{The order of cleaning antipatterns impacts the size of training data.} Figure~\ref{fig.orders.size} shows the distribution of different sizes from the data orders generated from 10-folds of training data from different project versions of the SDP data.\\
The position of class overlap impacts the data size more than the position of transformation and filtering. For instance, OMFT and OMTF with change in the order of filter-transform, have similar data sizes of median 603 and 613 respectively. This is in contrast to the positioning of mislabel with class overlap- \texttt{MOTF} has the medium of 1030.5 data points (largest of all groups). \\
Overall, cleaning mislabels before performing class overlap increases the data size. 
Figure~\ref{fig.orders.size} is plotted based on ascending median value of each cleaning order. The first six orders in Figure~\ref{fig.orders.size} have mislabels corrected after class overlap, whereas the last six orders that have larger training data sizes have class overlapped performed on the corrected labels. The overall comparison is statistically significant with Friedman test $p-value <= 0.05$.



==> old/rq2_orders-OLD.tex <==
 % experiment performe here: Results/skott_knott_Orders.py
 
\subsection{\rqtwoone}

\begin{figure}[!h]
      \hspace{-0.7cm}
      % \centering
      \includegraphics[width=1.2\columnwidth, keepaspectratio]{Images/orders_approach.drawio.pdf}
      \caption{Experiment setup for checking the impact of cleaning orders for various antipatterns.}
      \label{fig.cleaningorder}
    \end{figure}


\noindent \textbf{\textit{Motivation.}} 
The data pre-processing phase in ML pipelines involves preparing the data for the downstream components of the pipeline as noted by Amershi et al~\cite{amershi2019software}. This includes cleaning, performing transformations, and more. It is a topic that has been widely studied and is outlined in our Section~\ref{sec.back}. While previous research has focused on cleaning methods for specific data quality issues, the prevalence of multiple antipatterns as identified in \textbf{RQ1} calls for the need to clean them. An important question thus arises: What is the order in which these issues should be cleaned?\\
The sequence in which data quality issues are addressed can significantly affect the data size and distribution used for training the ML model. For example, removing instances of overlapped classes can decrease the size of the training data to a median of 17\%. This raises questions about the impact of removing the 17\% of data points on other antipatterns, such as correlated and redundant features, that may be addressed later. Additionally, had correlated and redundant features been removed first, this raises questions about the accuracy of the data representation- i.e., whether any information which could have been used to identify overlapping classes was lost. We aim to answer such questions by analyzing the model performance from different antipatterns in this RQ.\\
Data scientists and engineers working with ML models may face similar questions and come up with a logical order of cleaning these antipatterns. Indeed, for our own use case, we identified such a ``logical'' order for the subsequent RQs. However, our logic for cleaning may not apply to other datasets, and we are unaware of whether our identified ``logical" order yields the best performance for ML models.
Hence, through this research, we wish to identify the impact of the order of cleaning antipatterns on the performance of ML models using the case study of the SDP. We aim to provide an empirical understanding for researchers and practitioners of the impact of the order of cleaning data quality issues when building ML models. \\

\noindent \textbf{\textit{Approach.}}
To understand the impact of orders of cleaning multiple antipatterns, we create different orders on the training dataset, and build ML models on different learners. An overview of this process is mentioned in Fig~\ref{fig.cleaningorder}. Below we explain each step in detail:
\begin{itemize}
    \item \textit{Creation of Antipattern Cleaning Orders.} In \textbf{RQ1} (\ref{subsec.RQ1}), we observed the prevalence of eight antipatterns in the SDP data. We group these eight antipatterns into four categories, namely, \textit{Filtering} (F), \textit{Transformations} (T), \textit{Class Overlap} (O), and \textit{Mislabeling} (M). The grouping of cleaning various antipatterns into these four categories is based on their respective type of cleaning. % also mentioned in Table~\ref{tabcleaning}.
    In particular, \textit{Filtering} involves removing schema violations, duplicated data, constant features, and correlated \& redundant features. \textit{Transformation} involves mutating two antipatterns, tailed and not-normal features by performing Log-transformation and Z-scoring respectively. \textit{Mislabel} cleaning includes label correction, and finally \textit{Class Overlap} removes the data points with overlapping classes. We keep \textit{Class Overlap} separate from other filtering-based cleanings because of \textit{Mislabeling} having an explicit impact on \textit{Class Overlap}, whereas no impact on other cleaning techniques like schema violations, or constant features. \\
    Next, we create permutations of the four cleaning types to access the impact of cleaning order on the model performance. From all the permutations of \textit{F, T, O} and \textit{M}, we exclude the permutations which lead to the same result. In particular, the positioning of \textit{M} at any step before \textit{O} does not matter. For instance, mislabel positioning before overlap, in the case of \textit{FTMO}, (i.e. \textit{FMTO}, or \textit{MFTO}) yields the same data. Similarly, mislabel correction after class overlapping (e.g., \textit{OFTM, OFMT, OMFT}) yields the same data as well. \\
    Overall, we obtain 12 permutations of \textit{F, T, M,} and \textit{O}, which are referred to as \texttt{cleaning orders} henceforth. These cleaning orders are: \texttt{FMOT, FOMT,  FTMO, FTOM, MOFT, OMFT, MOTF, OMTF, TFMO, TFOM, TMOF, TOMF}. 
    
    \item \textit{Creation of ML pipelines.} We split the data into 80\% training and 20\% testing for validation purposes for each of the 12 cleaning orders and we use the same training data from the initial split to build 12 pipelines. Next, for each pipeline, we preprocess the respective training data according to its respective order, build a hyperparameter-tuned ML model, and finally, test the model against the unseen test set. While the base testing dataset is the same for the 12 pipelines, the same transformations (i.e., Log and Z-scoring) are performed on the testing set, as performed for the respective training set. This is done because the validation infrastructure has the same transformations as that of the training infrastructures~\cite{bhatia2022towards,amershi2019software}.
    
    \item \textit{Metric Evaluation.} To evaluate the impact of cleaning orders, we generate the six model metrics (i.e., AU-ROC, AU-PRC, F1, PR, RE, MCC) on each of the tests sets from the 10 data splits from each of the 12 cleaning orders.\\
    As described in Section~\ref{sec.casestudy}, we repeat the process for four learners and finally rank the metrics. We use the Scott-Knott Effect Size Difference (SK-ESD) test with $\alpha=0.05$~\cite{tantithamthavorn2016empirical}. The ESD  is an effect-aware variant of the traditional Scott Knott test, which uses hierarchical clustering to partition different sets of data means into statistically distinct groups.
\end{itemize}
\noindent \textbf{\textit{Results.}}

% threshold dep metrics
As depicted in Figure~\ref{fig.orders.auroc}, the orders \texttt{MOFT} and \texttt{MOTF} show high scores for all threshold-dependent metrics.  The order \texttt{MOFT} achieved the best F1, MCC, and Precision ranks among all learners and the best Recall rank for three out of four learners. However, the ranks of different learners show high inconsistency for a given threshold-dependent metric. For instance, the order \texttt{TMOF} has the highest precision rank for 50\% of the learners but the lowest rank for the remaining 50\%. This inconsistency is also seen in Precision, Recall, F1, and MCC metrics.
% AUC
The order \texttt{TMOF} has the best \textbf{AU-ROC} score, as shown by low ranks across all four learners. Other orders with mislabel correction before removing class overlapped rows (e.g., orders \texttt{MO: TFMO, FTMO}) also result in better AU-ROC scores for three out of four learners. Interestingly, out of all cleanings, starting with removal of class overlapped rows (i.e., order \texttt{MOFT}) resulted in the worst AU-ROC scores for all learners. This suggests that the distribution in the feature space used to identify overlapping classes should resemble the data used to build the models.
% AU prc
In the Figure~\ref{fig.orders.auprc}, the orders that performed mislabel correction after class overlap (\texttt{OMTF, FTOM, OMFT,} and \texttt{TFOM}) yielded higher AU-PRC scores, as indicated by their lowest ranks in all four learners. This suggests that class overlap correction having incorrect information about the response label improved the AU-PRC scores. However, these same orders had high AU-ROC ranks, indicating a inconsistency between the two metrics.
In fact, such inconsistencies between metric rankings are not just prevalent for AU-ROC and AU-PRC. \textbf{There is low concordance in ranks from different metrics for three out of four learners}. The Kendall's W level of concordance between ranks for different metrics was low ($W\leq0.3$) indicating that the order of cleaning antipatterns impacts different metrics differently. The values for Kendall's W for RF, DNN, and XGB are 0.29, 0.28, and 0.2 respectively, however, for LR the concordance is high (0.64).


%%%%%%%%---------------- FIG 4 AUROC
\begin{figure}[H]
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\columnwidth, keepaspectratio]{Images/ORDERS_AU-ROC.pdf}
\caption{Ranks for different orders of the Area Under Receiver Operator Curve metric.}
\label{fig.orders.auroc}
\end{subfigure}
%%%%%%%%---------------- FIG 4 AUPRC
\begin{subfigure}{\textwidth}
\includegraphics[width=\columnwidth, keepaspectratio]{Images/ORDERS_AU-PRC.pdf}
\caption{Ranks for different orders of the Area Under Precision-Recall metric.}
\label{fig.orders.auprc}
\end{subfigure}
%%%%%%%%---------------- FIG 4 F1
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\columnwidth, keepaspectratio]{Images/ORDERS_F1.pdf}
\caption{Ranks for different orders of the F1 score metric.}
\label{fig.orders.f1}
\end{subfigure}
%%%%%%%%---------------- FIG 4 MCC
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\columnwidth, keepaspectratio]{Images/ORDERS_MCC.pdf}
\caption{Ranks for different orders of the Mathews Correlation Coefficient metric.}
\label{fig.orders.mcc}
\end{subfigure}
%%%%%%%%---------------- FIG 4 PR
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\columnwidth, keepaspectratio]{Images/ORDERS_Precision.pdf}
\caption{Ranks for different orders of the Precision metric.}
\label{fig.orders.pr}
\end{subfigure}
%%%%%%%%---------------- FIG 4 RE
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\columnwidth, keepaspectratio]{Images/ORDERS_Recall.pdf}
\caption{Ranks for different orders of the Recall metric.}
\label{fig.orders.re}
\end{subfigure}
\caption{The threshold independent metrics (\ref{fig.orders.auprc}, \ref{fig.orders.auroc}) are shown in the gray color, whereas the threshold dependent metrics (\ref{fig.orders.f1}, \ref{fig.orders.mcc}, \ref{fig.orders.pr}, \ref{fig.orders.re}) are shown in the blue color. The cleaning orders presented in the x-axis are randomly ordered, but are consistent across all metrics.}
\end{figure}




\begin{Summary}{Summary of RQ2}{}
The order of cleaning antipatterns affects learner performance metrics differently. The highest ranks for threshold-dependent metrics are achieved by the orders \texttt{MOFT} and \texttt{MOTF}. Other orders show inconsistent results based on the metric. The AU-ROC metric has less variation than other metrics when antipatterns are cleaned using different orders. Correcting the response label information used for the class overlap correction improves AU-ROC scores but lowers the AU-PRC scores.
\end{Summary}

